Correcting Data Imbalance for Semi-Supervised Covid-19 Detection Using X-ray Chest Images

The Corona Virus (COVID-19) is an internationalpandemic that has quickly propagated throughout the world. The application of deep learning for image classification of chest X-ray images of Covid-19 patients, could become a novel pre-diagnostic detection methodology. However, deep learning architectures require large labelled datasets. This is often a limitation when the subject of research is relatively new as in the case of the virus outbreak, where dealing with small labelled datasets is a challenge. Moreover, in the context of a new highly infectious disease, the datasets are also highly imbalanced,with few observations from positive cases of the new disease. In this work we evaluate the performance of the semi-supervised deep learning architecture known as MixMatch using a very limited number of labelled observations and highly imbalanced labelled dataset. We propose a simple approach for correcting data imbalance, re-weight each observationin the loss function, giving a higher weight to the observationscorresponding to the under-represented class. For unlabelled observations, we propose the usage of the pseudo and augmentedlabels calculated by MixMatch to choose the appropriate weight. The MixMatch method combined with the proposed pseudo-label based balance correction improved classification accuracy by up to 10%, with respect to the non balanced MixMatch algorithm, with statistical significance. We tested our proposed approach with several available datasets using 10, 15 and 20 labelledobservations. Additionally, a new dataset is included among thetested datasets, composed of chest X-ray images of Costa Rican adult patients

==> images/gammas_semi_supervised.tex <==

\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100} 
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800} 
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500} 
 
\begin{tikzpicture}

\begin{axis}[ 
width=2.8in,
height=1.5in,
at={(0.758in,0.481in)},
scale only axis,
xmin=0,
xmax=50,
xlabel style={font=\color{white!15!black}},
xlabel={epochs},
ymin=-0.2,
ymax=1.2,
ylabel style={font=\color{white!15!black}},
ylabel={validation loss - training loss},
axis background/.style={fill=white}
]
\addplot [color=mycolor1, forget plot]
  table[row sep=crcr]{ 
1	-0.0146\\
2	-0.020491\\
3	-0.03454\\
4	-0.044948\\
5	-0.062871\\
6	-0.052588\\
7	-0.038852\\
8	0.022283\\
9	0.026367\\
10	0.06267\\
11	0.115013\\
12	0.337518\\
13	0.279202\\
14	0.461939\\
15	0.353554\\
16	0.620365\\
17	0.609262\\
18	0.629245\\
19	0.613158\\
20	0.79819\\
21	1.047408\\
22	0.756289\\
23	0.574803\\
24	0.74969\\
25	0.645984\\
26	0.669029\\
27	0.851897\\
28	0.761453\\
29	0.530914\\
30	0.88912\\
31	0.789673\\
32	0.776789\\
33	0.684963\\
34	0.679344\\
35	0.69154\\
36	0.58183\\
37	0.557511\\
38	0.558497\\
39	0.630093\\
40	0.635165\\
41	0.687109\\
42	0.670695\\
43	0.708623\\
44	0.703533\\
45	0.635898\\
46	0.733276\\
47	0.597587\\
48	0.542269\\
49	0.552185\\
50	0.523775\\
};
\addplot [color=mycolor2, forget plot]
  table[row sep=crcr]{ 
1	-0.020083\\
2	-0.034828\\
3	-0.041414\\
4	-0.068994\\
5	-0.082315\\
6	-0.084936\\
7	-0.065327\\
8	-0.032903\\
9	0.028245\\
10	0.015418\\
11	0.077941\\
12	0.190544\\
13	0.127146\\
14	0.195211\\
15	0.325694\\
16	0.495453\\
17	0.262646\\
18	0.407664\\
19	0.537773\\
20	0.530011\\
21	0.313609\\
22	0.408531\\
23	0.270102\\
24	0.78842\\
25	0.351807\\
26	0.482898\\
27	0.441483\\
28	0.412448\\
29	0.591506\\
30	0.492576\\
31	0.28587\\
32	0.410771\\
33	0.445066\\
34	0.397029\\
35	0.494835\\
36	0.351631\\
37	0.372128\\
38	0.435879\\
39	0.414524\\
40	0.440662\\
41	0.405002\\
42	0.460846\\
43	0.490234\\
44	0.449108\\
45	0.428192\\
46	0.459276\\
47	0.514107\\
48	0.456163\\
49	0.394698\\
50	0.47609\\
};
\addplot [color=mycolor3, forget plot]
  table[row sep=crcr]{ 
1	-0.013997\\
2	-0.021594\\
3	-0.019749\\
4	-0.026452\\
5	-0.017474\\
6	0.015677\\
7	0.016196\\
8	0.028161\\
9	0.065555\\
10	0.130449\\
11	0.150553\\
12	0.216045\\
13	0.263967\\
14	0.355523\\
15	0.358838\\
16	0.38597\\
17	0.422147\\
18	0.265475\\
19	0.536938\\
20	0.275884\\
21	0.860152\\
22	0.311852\\
23	0.392896\\
24	0.647758\\
25	0.641321\\
26	0.39052\\
27	0.357822\\
28	0.549876\\
29	0.481288\\
30	0.626727\\
31	0.37369\\
32	0.436187\\
33	0.408156\\
34	0.380425\\
35	0.553106\\
36	0.411105\\
37	0.426608\\
38	0.415271\\
39	0.519741\\
40	0.344306\\
41	0.333286\\
42	0.478583\\
43	0.406547\\
44	0.468316\\
45	0.433531\\
46	0.410427\\
47	0.406669\\
48	0.451838\\
49	0.440662\\
50	0.315889\\
};
\end{axis}
\end{tikzpicture} 


